Graph Partial Label Learning with Potential Cause Discovering

Graph Neural Networks (GNNs) have garnered widespread attention for their potential to address the challenges posed by graph representation learning, which face complex graph-structured data across various domains. However, due to the inherent complexity and interconnectedness of graphs, accurately annotating graph data for training GNNs is extremely challenging. To address this issue, we have introduced Partial Label Learning (PLL) into graph representation learning. PLL is a critical weakly supervised learning problem where each training instance is associated with a set of candidate labels, including the ground-truth label and the additional interfering labels. PLL allows annotators to make errors, which reduces the difficulty of data labeling. Subsequently, we propose a novel graph representation learning method that enables GNN models to effectively learn discriminative information within the context of PLL. Our approach utilizes potential cause extraction to obtain graph data that holds causal relationships with the labels. By conducting auxiliary training based on the extracted graph data, our model can effectively eliminate the interfering information in the PLL scenario. We support the rationale behind our method with a series of theoretical analyses. Moreover, we conduct extensive evaluations and ablation studies on multiple datasets, demonstrating the superiority of our proposed method.

==> Note.tex <==
2024.4.1
1. 确认一下all in one的数据集构成
2. 查找异质图数据集，难度越大越好，同时需要包括文本信息，进行列出
3. 实现方法，基于大模型进行节点特征生成以及节点属性生成, 之后融合图神经网络

2024.5.14
1. 实现如下算法模型：
    输入：节点特征为文本的异构图
    输出：节点分类、图分类、等
    1. 基于大模型将异构图的节点文本属性处理为向量特征，节点文本无-固-定-格-式。例如，如果节点文本可能为“这是一个原子节点，原子为氢原子”，也可能简单的为“H”。因此在处理向量特征的时候，需要使用如下prompt进行节点特征的处理：
       “对于节点描述“XXXXXX”，已知该描述是关于分子中一个原子的描述，请给出你对该描述的
       1）描述内容理解、
       2）描述的内容在原子中属于什么类型，（是关于原子属性的描述还是关于原子序号的描述？）、% 这里的问题个数还可以增加
       3）你对于你的评估有几分把握？，以如下格式输出：
       【关于问题1的答案】，【关于问题2的答案】，【关于问题3的答案】 
       同时注意每个答案的输出不要超过100字
       ”
    处理后，识别】与逗号符号将几个答案分开，变成答案1（内容）、答案2（类型）、答案3（可信度），然后对应去找它们的向量特征，即特征1（内容），特征2（类型），特征3（可信度），这些向量统一维度（长一点），不足就补0。处理不好的话，分开问也可以，另外prompt自己再优化下，主要的idea思想要体现。
    2. GNN处理，生成预测（节点分类、图分类等），具体生成方法如下：
        节点分类 = MLP（特征2（类型））   # 节点分类是一个代表类别标签的one-hot向量
        节点分类 = 节点分类与可信度交互处理，如果可信度低就soft一点，即让one-hot向量中的1小一点，其它值大一点点，这里具体使用啥公式自己选择一下

        # GNN layer 1：
        基于节点分类选择的权重 = 节点分类 x 权重矩阵 
        节点表示 = 特征1（内容）X 权重矩阵 
        节点表示 = 节点表示 x 基于节点分类选择的权重（三维的）
        正常进行一层GNN计算

        # GNN layer 2：
        基于节点分类选择的权重 = 节点分类 x 权重矩阵
        节点表示 = 特征1（内容）X 权重矩阵
        节点表示 = 节点表示 x 基于节点分类选择的权重（三维的）
        正常进行一层GNN计算

        ...

        输出预测
    3. 反向传播，训练

6.14
1.就是在GNN每一层里面价格可训练的B偏置，值可以很小，然后这个偏置也按照大模型判断的分类进行区分

2024.6.17 
1. 实现如下新的算法模型：
    输入：节点特征为文本的异构图
    输出：节点分类、图分类、等
    1. （本次新加入的模块）初始化异质节点的分类类型，使用大模型在不清楚分类种数的情况下，直接基于数据，自己分析出有哪几种类别。以IMDB数据集举例，按照数据集已经给出的信息，获取数据可以分为哪几种类别，使用大模型进行，进行如下提问：
       已知描述；“
       1.Mike Kaven，75000，3， 1 % 随机选取的训练集中第1条数据
       2.XXX，% 随机选取的训练集中第2条数据
       3.XXX，% 随机选取的训练集中第3条数据
       4.XXX，% 随机选取的训练集中第4条数据
       5.XXX  % 随机选取的训练集中第5条数据
       ...
       ”，这些描述可以分为哪三种类别？给出类别名称，名称不要超过5个字 % 注意此处的种类数量（这里为三种）为超参数
       回答如下：电影导演、电视导演、戏剧导演 
    2. 基于大模型将异构图的节点文本属性处理为向量特征，节点文本无-固-定-格-式。例如，如果节点文本可能为“这是一个关于导演Mike信息的描述”，也可能简单的为“Mike”。因此在处理向量特征的时候，需要使用如下prompt进行节点特征的处理：
       “对于节点描述“XXXXXX”，已知该描述是关于分子中一个原子的描述，请给出你对该描述的
       1）描述内容理解 
       2）提供内容所属于的类别，
       3）（本次新加入的模块）说明问题2的分析原因，分析与原因要区分开 
       4）（本次新加入的模块）描述的内容对于分类为XXX、XXX、XXX有何种影响，即分类为几个ground-truth类别的影响是什么，让大模型估计该特征数据 
       5）你对于你的评估有几分把握？
       答案以如下格式输出：
       【关于问题1的答案】，【关于问题2的答案】，【关于问题3的答案】 , ...
       同时注意每个答案的输出不要超过100字 
       ”
    处理后，识别】与逗号符号将几个答案分开，变成答案1（内容）、答案2（类型）、答案3（可信度），然后对应去找它们的向量特征，即特征1（内容），特征2（类型），特征3（可信度），这些向量统一维度（长一点），不足就补0。处理不好的话，分开问也可以，另外prompt自己再优化下，主要的idea思想要体现。即要体现LLM指导GNN针对不同类别节点表示使用不同权重，LLM的能力得到充分挖掘，LLM prompt要新颖有创新点 
    （本次新加入的模块）特征的生成，加入上面新生成的特征，包括内容所属于的类别分析原因，描述的内容对于分类为XXX、XXX、XXX有何种影响 
    3. GNN处理，生成预测（节点分类、图分类等），具体生成方法如下：
        节点分类 = MLP（特征2（类型））   # 节点分类是一个代表类别标签的one-hot向量
        节点分类 = 节点分类与可信度交互处理，如果可信度低就soft一点，即让one-hot向量中的1小一点，其它值大一点点，这里具体使用啥公式自己选择一下

        # GNN layer 1：
        基于节点分类选择的权重 = 节点分类 x 权重矩阵 
        节点表示 = 特征1（内容）X 权重矩阵 
        节点表示 = 节点表示 x 基于节点分类选择的权重（三维的）+ 基于节点分类选择的bias 
        （本次新加入的模块）确保可信度作为权重参数乘进去，这个自己咋实现都行，乘进去就成 
        正常进行一层GNN计算 

        # GNN layer 2：
        基于节点分类选择的权重 = 节点分类 x 权重矩阵 
        节点表示 = 特征1（内容）X 权重矩阵 
        节点表示 = 节点表示 x 基于节点分类选择的权重（三维的）+ 基于节点分类选择的bias 
        正常进行一层GNN计算 

        ...

        输出预测
    4. 反向传播，训练

2024.6.24 
    % 给出随机互联网选取的信息，进行分析
    % 进行少量的训练，就可以快速适应目标任务

2024.7.20
实验计划：
    1. 完成imdb等3个数据集实验实验，包括4种heterogeneous方法 加/不加 异构标签，OFA方法，纯GCN和GAT和方法，注意每个数据集需要计算两种metric，以及设定3种不同training/testing划分，（这里看下百分之五的training数据结果如何，如果表现好就加上百分之五，不好就不要）
    2. 完成两个新加数据集的实验（为IMDb与DBLP数据集的增强版，让节点信息更加混乱，该实验加入所谓的对其MLP层，就是做两次node type划分，第一层是划分数据形式，第二层是划分节点属性类型），两个新加数据集分析两组，纯新加数据，与新加数据与原始数据混合两种，也需要计算两种metric
    3. 完成1个非heterogeneous数据集上的实验，baseline还是以上那些
    4. 完成消融实验，分别去掉我们对GNN中的3中改动，观察模型表现，只在一个数据集上进行这个实验即可
    5. 完成对比实验，比较我们的方法所划分标签与实际标签之间的区别，给出10个实际节点的分类实例，以及对于数据集中，我们方法正确划分的比例
    6. 使用t-SNE方法，可视化我们方法对于所有数据集特征类别，每个类别一个颜色，记得把最终输出的特征（过MLP进行分类前的），以及从LLM中得到的那个特征都弄一下，这样可以对比下我们方法中的GNN起了啥作用。
    7. 每个数据集给出5个比较好的我们的算法的LLM的节点特征分析的输出，文字版本，转为特征向量之前的
    8. 逐渐加大IMDB（DBLP也行）中，我们的生成的新的混乱节点信息的比例，观察我们的方法的表现和1种heterogeneous方法baseline的比较
    
